On the Formalization of Cryptographic Migration

We present a novel approach to gaining insight into the structure of cryptographic migration problems which are classic problems in applied cryptography. We use a formal model to capture the inherent dependencies and complexities of such transitions. Using classical mathematical results from combinatorics, probability theory, and combinatorial analysis, we evaluate the challenges of migrating large cryptographic IT infrastructures and prove that - in a suitable sense - cryptographic migration exhibits a certain expected complexity. We also provide numerical data for selected parameter sets. Furthermore, we analyze the proposed model in terms of real-world patterns and its practical applicability. Additionally, we discuss the challenges of modeling real-world migration projects. As concrete examples we examine the transition to post-quantum cryptography of the CI/CD system GitLab and the multi-level technological transition of distribution power grids. This work paves the way for future advancements in both the theoretical understanding and practical implementation of cryptographic migration strategies.

==> sections/power-grid-ict.tex <==
%We could use an example CI to show that we can establish migration graphs on different levels of abstractions (possibly called views?); we take a high-level infrastructure view and show a graph and its migration clusters (along with patterns) there and then take one of the subsystems and analyse it again in the same way; we can also discuss how a migration cluster can be wrapped, e.g., by using VPN or similar

As an example of critical infrastructure, we are going to discuss modern power distribution grids. Power grids are a critical infrastructure in any modern society and have been the target of cyber attacks, e.g., in the war between Russian and Ukraine\footnote{\url{https://en.wikipedia.org/wiki/2015_Ukraine_power_grid_hack}}. The increased digitalisation and the move towards more sophisticated monitoring infrastructure deployed in the grid in a distributed fashion open many new attack paths~\cite{tatipatri2024comprehensive}. Tatipatri and Arun~\cite{tatipatri2024comprehensive} provide a taxonomy of possible attacks, ranging from injecting false data into measurement system to physical attacks on the equipment. Generally, the aim of such attacks is to disrupt the service of the power system and stop the flow of power to consumers, often by destroying the power equipment itself.

There are a number of standards that describe the architectures, protocols, and security measures used in power distribution grids. IEC 61968 defines protocols used in the communication between power equipment. IEC 62351 defines technical aspects of cyber-security for securing process data communication in power systems. Here,  IEC 61580 defines the ICT architecture of a substation based on Ethernet. Together, these standards provide comprehensive guidelines on how to secure parts of the power system. At their core, they all rely on cryptography to authenticate and authorize access to the systems and encrypt and verify the information that is exchanged between the components.

\subsubsection{Architecture of the Power Distribution Grid}

The power distribution grid is organised as a layered system. These layers often correspond to voltage levels. In the following, we will use a somewhat simplified architecture, as the actual power flows are not relevant in our analysis of the ICT architecture.

The role of the power distribution grid is to bring stepped-down power to the consumers. While there are some smaller power generators (such as smaller solar forms or individual wind turbines) are connected to the distribution grid, the flow of power is mostly from the high-voltage transmission grid into the medium- and low-voltage distribution grids. Electrical substations contain transformers to convert the voltages. Community-scale solar farms and larger industrial and commercial consumers are directly connected to such substations. Smaller consumers are connected via distributed transformers that step down the voltage to the levels required for residential or small commercial consumers.

All of the mentioned elements are connected to an information system. Residential and small commercial consumers have smart meters that communicate, e.g., via power-line communication (PLC) or the internet. Metered transformers that can be installed on power poles connect via mobile phone networks or microwave communication. Power poles can also be equipped with remotely-controlled reclosers, i.e., large power switches. Larger consumers have dedicated hardware that monitors the power quality (voltage, current, frequency, waveform distribution) and often have remotely-controlled breakers as well. Distribution substations have feeder meters and equipment to control the power quality and are largely controllable remotely. Large consumers and substations are either connected with wired connections or via 4G networks. There is a trend towards an even more more distributed systems with a number of edge devices to provide even more detailed situational awareness and enable some distributed control~\cite{rehtanz2024towards}.

The information generated by all of this equipment is collected and analysed in the operations center of a distribution grid provider. The operators there can observe the status of different grid areas and take control actions, such as disconnecting a grid area if necessary. This centralized control is done using SCADA (Supervisory Control and Data Acquisition) systems, which consist of hardware and software that allow organizations to monitor and control the power equipment remotely. Figure~\ref{fig:distribution-grid-architecture} shows a simplified schematic of such a system.

\begin{figure}
    \includegraphics[width=\columnwidth]{pictures/distribution-grid-architecture.pdf}
    \caption{A schematic view of the elements that are relevant on the infrastructure level of the distribution grid. Solid lines represent the energy network, dotted lines the communication network.}
    \label{fig:distribution-grid-architecture}
\end{figure}

\subsubsection{A Migration Graph for the Infrastructure Level}

Where we describe what a migration on the infrastructure level would look like.

\subsubsection{Architecture of a Smart Distribution Substation}

Where we describe which components a substation is composed of.

\begin{figure}
    \includegraphics[width=\columnwidth]{pictures/substation-architecture.pdf}
    \caption{A rough overview of the ICT architecture of a distribution substation based roughly o ~\cite{chattopadhyay2017toward}. Sensors are connected to intelligent electronic devices (IEDs) which in turn are connected to teh substation automation system via Ethernet using High-availability Seamless Redundancy (HSR) and Parallel Redundancy Protocol (PRP). In some cases, IEDs are first connected to remote terminal units (RTU) which are then connected to the automation system. The protocols used are based on IEC~61580. Please note that an actual system would contain redundant automation, RTUs, and IEDs for some aspects.}
    \label{fig:substation-architecture}
\end{figure}

\cite{hussain2019review} describes the security mechanisms defined in IEC 62351.

\subsubsection{A Migration Graph for a Distribution Substation}

Where we describe what a migration of a distribution substation would look like.

\subsubsection{Substation Automation System}

Where we describe what the SCADA system within a substation looks like.

\subsubsection{A Migration Graph for the Substation Automation System}

Where we describe what a migration of a substation automation system would look like.

\subsubsection{Combining the Three Levels}

Where we describe what we learn when we do the decomposition of the migration graph.
